How should we select test-negative controls? A causal perspective in the era of multiplex respiratory testing

The test-negative design (TND) is widely used to estimate vaccine effectiveness (VE) for respiratory pathogens by comparing vaccination odds among test-positive cases versus test-negative controls. A central yet underexplored design element is which test-negative illnesses constitute valid controls. With rapid multiplex PCR panels, investigators can now identify specific non-focal pathogens among test-negative patients, allowing for better characterization of ``test-negative illness'', but also revealing a mixture of control outcomes that may each satisfy or violate causal assumptions. We synthesize recent causal identification results for the TND and show that they imply two distinct interpretations of control selection: 1) a sampling view in which controls represent the source population and 2) a bias-correction view in which controls function as negative control outcomes under equi-confounding. Building on these interpretations, we develop a framework for multiplex-informed control selection. We propose a taxonomy that distinguishes controls that serve primarily as exposure proxies (sharing unmeasured determinants of infection) from those that serve as testing proxies (sharing unmeasured determinants of care-seeking), derive implications for pathogen-specific and pooled estimators, and suggest three practical principles for control selection: vaccine irrelevance, avoidance of entanglement with other interventions, and testing-process comparability. We also formalize nuances introduced by multiplex panels, including co-detections and pan-negative episodes, and outline when standard pooled estimators remain valid versus when alternative estimators are needed. In simulations across 9 scenarios, we demonstrate violations concentrated in a single control pathogen can substantially bias pooled TND estimates, whereas a pre-specified pathogen screening estimator remained unbiased.

==> results/tables/prevalence_sweep.tex <==
\begin{table}[ht]
\centering
\caption{Bias and root mean squared error (RMSE) of TND estimators by control pathogen prevalence across three violation scenarios. Bias and RMSE are expressed in percentage points (pp). SE denotes the Monte Carlo standard error of the mean bias.}
\label{tab:prevalence_sweep}
\begin{tabular}{llrrrr}
\toprule
Scenario & Estimator & Prev. (%) & Bias (pp) & RMSE (pp) & SE \\
\midrule
At-home testing differential & Pooled TND & 11 & -6.3 & 10.0 & 0.35 \\
At-home testing differential & Pooled TND & 14 & -6.9 & 10.6 & 0.36 \\
At-home testing differential & Pooled TND & 17 & -8.1 & 11.4 & 0.36 \\
At-home testing differential & Pooled TND & 2 & -1.7 & 7.2 & 0.31 \\
At-home testing differential & Pooled TND & 20 & -9.2 & 12.2 & 0.36 \\
At-home testing differential & Pooled TND & 23 & -10.2 & 13.0 & 0.36 \\
At-home testing differential & Pooled TND & 5 & -3.5 & 8.1 & 0.33 \\
At-home testing differential & Pooled TND & 8 & -4.3 & 8.5 & 0.33 \\
At-home testing differential & Screened TND & 11 & -0.7 & 7.1 & 0.32 \\
At-home testing differential & Screened TND & 14 & -0.2 & 7.4 & 0.33 \\
At-home testing differential & Screened TND & 17 & -0.3 & 7.1 & 0.32 \\
At-home testing differential & Screened TND & 2 & -0.5 & 7.1 & 0.31 \\
At-home testing differential & Screened TND & 20 & -0.5 & 7.2 & 0.32 \\
At-home testing differential & Screened TND & 23 & -0.5 & 7.1 & 0.32 \\
At-home testing differential & Screened TND & 5 & -0.6 & 7.1 & 0.32 \\
At-home testing differential & Screened TND & 8 & +0.0 & 6.9 & 0.31 \\
\addlinespace
Other-vaccine entanglement & Pooled TND & 11 & -2.6 & 7.6 & 0.32 \\
Other-vaccine entanglement & Pooled TND & 14 & -3.2 & 8.1 & 0.33 \\
Other-vaccine entanglement & Pooled TND & 17 & -3.7 & 8.1 & 0.32 \\
Other-vaccine entanglement & Pooled TND & 2 & -0.9 & 6.9 & 0.31 \\
Other-vaccine entanglement & Pooled TND & 20 & -4.0 & 7.8 & 0.30 \\
Other-vaccine entanglement & Pooled TND & 23 & -4.8 & 9.0 & 0.34 \\
Other-vaccine entanglement & Pooled TND & 5 & -1.6 & 7.2 & 0.32 \\
Other-vaccine entanglement & Pooled TND & 8 & -2.2 & 7.3 & 0.31 \\
Other-vaccine entanglement & Screened TND & 11 & -0.2 & 7.1 & 0.32 \\
Other-vaccine entanglement & Screened TND & 14 & -0.3 & 7.1 & 0.32 \\
Other-vaccine entanglement & Screened TND & 17 & -0.5 & 7.1 & 0.32 \\
Other-vaccine entanglement & Screened TND & 2 & -0.2 & 6.8 & 0.30 \\
Other-vaccine entanglement & Screened TND & 20 & -0.2 & 6.4 & 0.28 \\
Other-vaccine entanglement & Screened TND & 23 & -0.6 & 7.3 & 0.33 \\
Other-vaccine entanglement & Screened TND & 5 & -0.2 & 6.9 & 0.31 \\
Other-vaccine entanglement & Screened TND & 8 & -0.4 & 6.9 & 0.31 \\
\addlinespace
Vaccine irrelevance violation & Pooled TND & 11 & -6.5 & 9.7 & 0.32 \\
Vaccine irrelevance violation & Pooled TND & 14 & -7.4 & 10.6 & 0.34 \\
Vaccine irrelevance violation & Pooled TND & 17 & -7.8 & 11.2 & 0.36 \\
Vaccine irrelevance violation & Pooled TND & 2 & -1.6 & 7.3 & 0.32 \\
Vaccine irrelevance violation & Pooled TND & 20 & -9.3 & 12.3 & 0.36 \\
Vaccine irrelevance violation & Pooled TND & 23 & -9.4 & 12.6 & 0.37 \\
Vaccine irrelevance violation & Pooled TND & 5 & -3.5 & 8.2 & 0.33 \\
Vaccine irrelevance violation & Pooled TND & 8 & -4.9 & 9.0 & 0.34 \\
Vaccine irrelevance violation & Screened TND & 11 & -0.5 & 6.7 & 0.30 \\
Vaccine irrelevance violation & Screened TND & 14 & -0.5 & 6.9 & 0.31 \\
Vaccine irrelevance violation & Screened TND & 17 & +0.1 & 7.2 & 0.32 \\
Vaccine irrelevance violation & Screened TND & 2 & -0.1 & 6.9 & 0.31 \\
Vaccine irrelevance violation & Screened TND & 20 & -0.4 & 7.1 & 0.32 \\
Vaccine irrelevance violation & Screened TND & 23 & -0.0 & 7.3 & 0.33 \\
Vaccine irrelevance violation & Screened TND & 5 & -0.4 & 7.1 & 0.32 \\
Vaccine irrelevance violation & Screened TND & 8 & -0.3 & 7.1 & 0.32 \\
\bottomrule
\end{tabular}
\\[0.5em]
\footnotesize{Note: Bias and RMSE are in percentage points (pp). SE = Monte Carlo standard error of the mean bias. Ribbons in the corresponding figures show $\pm 1.96 \times$ SE.}
\end{table}


==> results/tables/violation_sweep.tex <==
\begin{table}[ht]
\centering
\caption{Bias and root mean squared error (RMSE) of TND estimators by violation magnitude across three violation scenarios. Bias and RMSE are expressed in percentage points (pp). SE denotes the Monte Carlo standard error of the mean bias. The violation strength parameter is scenario-specific: cross-protection log-OR (vaccine irrelevance), U-coupling coefficient (entanglement), or at-home testing probability gap (at-home testing).}
\label{tab:violation_sweep}
\begin{tabular}{llrrrr}
\toprule
Scenario & Estimator & Strength & Bias (pp) & RMSE (pp) & SE \\
\midrule
At-home testing differential & Pooled TND & 0.00 & -0.5 & 7.5 & 0.33 \\
At-home testing differential & Pooled TND & 0.10 & -1.0 & 6.9 & 0.31 \\
At-home testing differential & Pooled TND & 0.20 & -1.5 & 7.4 & 0.32 \\
At-home testing differential & Pooled TND & 0.30 & -2.5 & 7.9 & 0.34 \\
At-home testing differential & Pooled TND & 0.40 & -3.0 & 7.5 & 0.31 \\
At-home testing differential & Pooled TND & 0.50 & -3.7 & 8.1 & 0.32 \\
At-home testing differential & Screened TND & 0.00 & -0.3 & 7.5 & 0.34 \\
At-home testing differential & Screened TND & 0.10 & -0.2 & 6.8 & 0.30 \\
At-home testing differential & Screened TND & 0.20 & -0.0 & 7.2 & 0.32 \\
At-home testing differential & Screened TND & 0.30 & -0.3 & 7.3 & 0.33 \\
At-home testing differential & Screened TND & 0.40 & -0.3 & 6.7 & 0.30 \\
At-home testing differential & Screened TND & 0.50 & -0.2 & 6.9 & 0.31 \\
\addlinespace
Other-vaccine entanglement & Pooled TND & 0.50 & -0.9 & 7.0 & 0.31 \\
Other-vaccine entanglement & Pooled TND & 1.00 & -0.6 & 7.1 & 0.32 \\
Other-vaccine entanglement & Pooled TND & 1.50 & -1.3 & 7.2 & 0.32 \\
Other-vaccine entanglement & Pooled TND & 2.00 & -1.3 & 7.7 & 0.34 \\
Other-vaccine entanglement & Pooled TND & 2.50 & -1.7 & 7.1 & 0.31 \\
Other-vaccine entanglement & Pooled TND & 3.00 & -1.5 & 7.3 & 0.32 \\
Other-vaccine entanglement & Screened TND & 0.50 & -0.5 & 7.0 & 0.31 \\
Other-vaccine entanglement & Screened TND & 1.00 & +0.1 & 7.1 & 0.32 \\
Other-vaccine entanglement & Screened TND & 1.50 & -0.4 & 7.0 & 0.31 \\
Other-vaccine entanglement & Screened TND & 2.00 & -0.3 & 7.5 & 0.34 \\
Other-vaccine entanglement & Screened TND & 2.50 & -0.7 & 6.9 & 0.31 \\
Other-vaccine entanglement & Screened TND & 3.00 & -0.4 & 7.1 & 0.32 \\
\addlinespace
Vaccine irrelevance violation & Pooled TND & -0.10 & -1.8 & 7.2 & 0.31 \\
Vaccine irrelevance violation & Pooled TND & -0.20 & -1.9 & 7.5 & 0.33 \\
Vaccine irrelevance violation & Pooled TND & -0.30 & -2.1 & 7.6 & 0.33 \\
Vaccine irrelevance violation & Pooled TND & -0.40 & -3.3 & 8.4 & 0.34 \\
Vaccine irrelevance violation & Pooled TND & -0.50 & -3.9 & 8.0 & 0.31 \\
Vaccine irrelevance violation & Pooled TND & -0.60 & -3.9 & 8.6 & 0.34 \\
Vaccine irrelevance violation & Pooled TND & -0.70 & -4.7 & 8.7 & 0.33 \\
Vaccine irrelevance violation & Pooled TND & 0.00 & -0.1 & 6.8 & 0.31 \\
Vaccine irrelevance violation & Screened TND & -0.10 & -0.9 & 7.0 & 0.31 \\
Vaccine irrelevance violation & Screened TND & -0.20 & -0.3 & 7.2 & 0.32 \\
Vaccine irrelevance violation & Screened TND & -0.30 & -0.1 & 7.2 & 0.32 \\
Vaccine irrelevance violation & Screened TND & -0.40 & -0.7 & 7.5 & 0.33 \\
Vaccine irrelevance violation & Screened TND & -0.50 & -0.7 & 6.8 & 0.30 \\
Vaccine irrelevance violation & Screened TND & -0.60 & -0.4 & 7.2 & 0.32 \\
Vaccine irrelevance violation & Screened TND & -0.70 & -0.7 & 7.1 & 0.32 \\
Vaccine irrelevance violation & Screened TND & 0.00 & +0.2 & 6.9 & 0.31 \\
\bottomrule
\end{tabular}
\\[0.5em]
\footnotesize{Note: Bias and RMSE are in percentage points (pp). SE = Monte Carlo standard error of the mean bias. Ribbons in the corresponding figures show $\pm 1.96 \times$ SE.}
\end{table}

